BEC: Bit-Level Static Analysis for Reliability against Soft Errors

Soft errors are a type of transient digital signal corruption that occurs in digital hardware components such as the internal flip-flops of CPU pipelines, the register file, memory cells, and even internal communication buses. Soft errors are caused by environmental radioactivity, magnetic interference, lasers, and temperature fluctuations, either unintentionally, or as part of a deliberate attempt to compromise a system and expose confidential data. We propose a bit-level error coalescing (BEC) static program analysis and its two use cases to understand and improve program reliability against soft errors. The BEC analysis tracks each bit corruption in the register file and classifies the effect of the corruption by its semantics at compile time. The usefulness of the proposed analysis is demonstrated in two scenarios, fault injection campaign pruning, and reliability-aware program transformation. Experimental results show that bit-level analysis pruned up to 30.04 % of exhaustive fault injection campaigns (13.71 % on average), without loss of accuracy. Program vulnerability was reduced by up to 13.11 % (4.94 % on average) through bit-level vulnerability-aware instruction scheduling. The analysis has been implemented within LLVM and evaluated on the RISC-V architecture. To the best of our knowledge, the proposed BEC analysis is the first bit-level compiler analysis for program reliability against soft errors. The proposed method is generic and not limited to a specific computer architecture.

==> implementation.tex <==
%LLVM provides a class called \emph{KnownBits} to analyze the contents of the bits at compile-time. The KnownBits class is designed to support LLVM IR which is target independent, and we extended the existing KnownBits class to support RISC-V specific instructions. The data flow of a program is concertized step-by-step during the compilation. The virtual registers of LLVM IR in SSA form are transformed into physical registers by register allocation, and data-flow of stack pointer or frame pointer are materialized once the usage of stacks slots are determined. The static result index collapsing can be performed only when the data-flows are exposed to the program. Thus the proposed bit-level analysis is performed just before the code emission when the most data-flows are realized.
%For the bit-level vulnerability-aware instruction scheduling, an additional run of the proposed analysis is performed before the machine instruction scheduling phase so the machine instruction scheduling pass can use the analysis result as the instruction scheduling criteria.

%Once the static result indexes are analyzed at the end of the compilation phase, the analysis result is emitted along with the codes in the form of comments so it does not affect the program itself. The static analysis results are passed on to the system that conducts the fault injection campaign. 

